Anisotropy of the interface tension of the three-dimensional Ising model

We determine the interface tension for the 100, 110 and 111 interface of the simple cubic Ising model with nearest-neighbour interaction using novel simulation methods. To overcome the droplet/strip transition and the droplet nucleation barrier we use a newly developed combination of the multimagnetic algorithm with the parallel tempering method. We investigate a large range of inverse temperatures to study the anisotropy of the interface tension in detail.

==> Makefile <==
.PHONY:all clean
	
LATEX=latex
DVIPS=dvips

SOURCES=interface.tex
EPS=fss_s100.eps  fss_s110.eps  fss_s111.eps  p_m_s100.eps  s100.eps  s110.eps  s111.eps ratio_2d_3d_v1.eps sigma_fit3.eps sigma_fit4.eps 
TOOLS=Makefile

all: $(SOURCES:.tex=.ps)

clean:
	rm -f *.aux *.log

.tex.dvi:
	$(LATEX) --interaction nonstopmode $< | clean_tex
	$(LATEX) --interaction nonstopmode $< | clean_tex
	/bin/kill -SIGUSR1 `ps -C xdvi.bin -o "%p" --no-heading`; true

%.ps: %.dvi
	$(DVIPS) $<

%.pdf: %.dvi
	$(DVIPDF) $<

tar:
	@D=`date '+%d_%m_%y'`; \
	tar -czf "interface_$${D}.tar.gz" $(SOURCES) $(EPS) $(TOOLS); 


